Optimal Prediction of Synchronization-Preserving Races

Concurrent programs are notoriously hard to write correctly, as scheduling nondeterminism introduces subtle errors that are both hard to detect and to reproduce. The most common concurrency errors are (data) races, which occur when memory-conflicting actions are executed concurrently. Consequently, considerable effort has been made towards developing efficient techniques for race detection. The most common approach is dynamic race prediction: given an observed, race-free trace $\sigma$ of a concurrent program, the task is to decide whether events of $\sigma$ can be correctly reordered to a trace $\sigma^*$ that witnesses a race hidden in $\sigma$. In this work we introduce the notion of sync(hronization)-preserving races. A sync-preserving race occurs in $\sigma$ when there is a witness $\sigma^*$ in which synchronization operations (e.g., acquisition and release of locks) appear in the same order as in $\sigma$. This is a broad definition that strictly subsumes the famous notion of happens-before races. Our main results are as follows. First, we develop a sound and complete algorithm for predicting sync-preserving races. For moderate values of parameters like the number of threads, the algorithm runs in $\widetilde{O}(\mathcal{N})$ time and space, where $\mathcal{N}$ is the length of the trace $\sigma$. Second, we show that the problem has a $\Omega(\mathcal{N}/\log^2 \mathcal{N})$ space lower bound, and thus our algorithm is essentially time and space optimal. Third, we show that predicting races with even just a single reversal of two sync operations is $\operatorname{NP}$-complete and even $\operatorname{W}[1]$-hard when parameterized by the number of threads. Thus, sync-preservation characterizes exactly the tractability boundary of race prediction, and our algorithm is nearly optimal for the tractable side.

==> abstract_bk.tex <==
%!TEX root = main.tex

\begin{abstract}
Concurrent programs are notoriously hard to write correctly, as scheduling nondeterminism introduces subtle errors that are both hard to detect and to reproduce.
The most common concurrency errors are \emph{(data) races}, which occur when memory-conflicting actions are executed concurrently.
Consequently, considerable efforts are made towards efficient techniques for race detection.
The most usual approach is \emph{dynamic race prediction}:~
given an observed, race-free trace $\tr$ of a concurrent program, the task is to decide whether events of $\tr$ can be correctly reordered to a trace $\tr^*$ that witnesses a race hidden in $\tr$.
 

In this work we introduce the notion of \emph{sync(hronization)-reversal free races}.
A sync-reversal free race occurs in $\tr$ when there is a witness $\tr^*$ 
in which synchronization operations (e.g., acquisition and release of locks)
appear in the same order as in $\tr$.
This is a broad definition that \emph{strictly subsumes} the famous notion of happens-before races.
Our main results are as follows.
First, we develop a \emph{sound and complete} algorithm for predicting sync-reversal free races that runs in $\Otilde(\NumEvents)$ time and space, for up to a moderate number of other parameters, such as the number of threads.
Second, we show that the problem has a $\Omega(\NumEvents/\log^2 \NumEvents)$ space lower bound, and thus our algorithm is essentially \emph{time and space optimal}.
Third, we show that predicting races with \emph{even just a single} reversal of two sync operations is $\NP$-complete and even $\W{1}$-hard when parameterized by the number of threads.
Thus, sync-reversal freeness characterizes \emph{exactly} the tractability boundary of race prediction, and our algorithm is nearly \emph{optimal} for the tractable side.
Our experiments show that our algorithm is fast in practice, while sync-reversal freeness characterizes races often missed by state-of-the-art methods.
\end{abstract}


%% 2012 ACM Computing Classification System (CSS) concepts
%% Generate at 'http://dl.acm.org/ccs/ccs.cfm'.
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10011007.10011074.10011099</concept_id>
<concept_desc>Software and its engineering~Software verification and validation</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003752.10010070</concept_id>
<concept_desc>Theory of computation~Theory and algorithms for application domains</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10003752.10010124.10010138.10010143</concept_id>
<concept_desc>Theory of computation~Program analysis</concept_desc>
<concept_significance>300</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Software and its engineering~Software verification and validation}
\ccsdesc[300]{Theory of computation~Theory and algorithms for application domains}
\ccsdesc[300]{Theory of computation~Program analysis}

%% End of generated code


%% Keywords
%% comma separated list
\keywords{concurrency, dynamic analysis, race detection, complexity}  %% \keywords are mandatory in final camera-ready submission

==> exec_macros.tex <==
%!TEX root = main.tex

% Drawing executions. Arguments: # of threads, and execution.
\newcommand{\execution}[2]{
\scalebox{0.85}{
  \begin{tikzpicture}%
    \foreach \x in {1,...,#1}
    \node[right] at (1.5*\x+0.2,0.25) {$t_{\x}$};
    \draw (1.2,0) -- (#1*1.5+1.3,0);%
    \pgfmathsetmacro{\y}{1};%
    #2%
    \draw (1.2,0) -- (1.2,-0.4*\y);%
    \draw (#1*1.5+1.3,0) -- (#1*1.5+1.3,-0.4*\y);%
    \foreach \x in {2,...,#1}
    % \draw[dashed] (1.5*\x-0.3,0) -- (1.5*\x-0.3,-0.4*\y);%
    \draw (1.2,-0.4*\y) -- (#1*1.5+1.3,-0.4*\y);%
  \end{tikzpicture}
}
}

% \figev arguments: thread id, event, variable/lock
\newcommand{\figev}[2]{
\pgfmathsetmacro{\y}{\y+1};
\pgfmathsetmacro{\y}{\y-1};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\y}};%
\node at (#1*1.5 + 0.45,-0.4*\y) {$ #2 $};%
\pgfmathsetmacro{\y}{\y+1};
}


\newcommand{\executionlarge}[2]{
\scalebox{0.85}{
  \begin{tikzpicture}%
    \foreach \x in {1,...,#1}
    \node[right] at (1.9*\x+0.2,0.25) {$t_{\x}$};
    \draw (1.2,0) -- (#1*1.9+1.9,0);%
    \pgfmathsetmacro{\y}{1};%
    #2%
    \draw (1.2,0) -- (1.2,-0.4*\y);%
    \draw (#1*1.9+1.9,0) -- (#1*1.9+1.9,-0.4*\y);%
    \foreach \x in {2,...,#1}
    % \draw[dashed] (1.5*\x-0.3,0) -- (1.5*\x-0.3,-0.4*\y);%
    \draw (1.2,-0.4*\y) -- (#1*1.9+1.9,-0.4*\y);%
  \end{tikzpicture}
}
}

% \figev arguments: thread id, event, variable/lock
\newcommand{\figevlarge}[2]{
\pgfmathsetmacro{\y}{\y+1};
\pgfmathsetmacro{\y}{\y-1};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\y}};%
\node at (#1*1.9 + 0.45,-0.4*\y) {$ #2 $};%
\pgfmathsetmacro{\y}{\y+1};
}


% \figev arguments: thread id, event, variable/lock, 3rd arg = event id offset

% \newcommand{\mathresult}[1]{\pgfmathparse{#1} \pgfmathresult}
% \newcommand{\addmathresult}[1]{\pgfmathparse{2 *\mathresult{#1}} \pgfmathresult}

\newcommand{\figevoffset}[3]{
\pgfmathparse{#1}
\pgfmathsetmacro{\offset}{\pgfmathresult};
\pgfmathparse{\y+\offset}
\pgfmathsetmacro{\newindex}{\pgfmathresult};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\newindex}};%
\node at (#2*1.5 + 0.45,-0.4*\y) {$ #3 $};%
\pgfmathsetmacro{\y}{\y+1};
}


%\orderedeg{t1}{ind1}{off1}{t2}{ind2}{off2} denotes an edge from an event e1
% to an event e2 such that ei appears at indi in the trace and belongs to thread ti.
% off1 and off2 are offsets from the center.
\newcommand{\orderedge}[6]{
  \draw (#1*1.5 + 0.45 + #3, -0.4*#2) edge[-{Latex[length=2mm, width=2mm]},  ->,>=stealth] (#4*1.5 + 0.45 + #6, -0.4*#5);
}

% The 7th arg is the label and the 8th argument is the position
\newcommand{\orderedgewithlabel}[8]{
  \draw (#1*1.5 + 0.45 + #3, -0.4*#2) edge[-{Latex[length=2mm, width=2mm]},  ->,>=stealth] node[anchor=center, sloped, #8] { #7} (#4*1.5 + 0.45 + #6, -0.4*#5);
}

\newcommand{\executionnonumber}[2]{\begin{tikzpicture}%
                             \foreach \x in {1,...,#1}
                               \node[right] at (2*\x+0.5,0.25) {$t_{\x}$};
                             \draw (1.9,0) -- (#1*2+1.6,0);%
                             \pgfmathsetmacro{\z}{1};%
                             #2%
                             \draw (1.9,0) -- (1.9,-0.5*\z);%
                             \draw (#1*2+1.6,0) -- (#1*2+1.6,-0.5*\z);%
                             \foreach \x in {2,...,#1}
                               \draw (2*\x-0.3,0) -- (2*\x-0.3,-0.5*\z);%
                             \draw (1.9,-0.5*\z) -- (#1*2+1.6,-0.5*\z);%
                           \end{tikzpicture}}                    

\newcommand{\figevnonumber}[2]{\node [left] at (1.75,-0.4*\z) {};%
\node [right] at (#1*2 + 0.3,-0.5*\z) {$ #2 $};%
\pgfmathsetmacro{\z}{\z+1};}

% Drawing programs. Arguments: # of threads, and program
\newcommand{\figprogram}[2]{\begin{tikzpicture}%
                              \foreach \x in {1,...,#1}
                                \node at (2.3*\x-1.15,0.25) {$t_{\x}$};
                              \draw (0,0) -- (#1*2.3+0.6,0);% 
                              \pgfmathsetmacro{\y}{1};%
                              #2%
                              \draw (0,0) -- (0,-0.4*\y);% 
                              \draw (#1*2.3+0.6,0) -- (#1*2.3+0.6,-0.4*\y);% 
                              \draw (0,-0.4*\y) -- (#1*2.3+0.6,-0.4*\y);% 
                            \end{tikzpicture}}
% figstmt arguments: thread id, offset, statement
\newcommand{\figstmt}[3]{\node [left] at (-0.15,-0.4*\y) {\pgfmathprintnumber{\y}};%
                      \node[right] at (#1*2.3 + #2*0.3 - 2.15,-0.4*\y) {\texttt{#3}};
                      \pgfmathsetmacro{\y}{\y+1};}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newtheorem{observation}{Observation}

\newcommand{\nil}{\texttt{nil}}

\newcommand{\drawarrow}{\raisebox{2pt}{\scalebox{0.7}{\tikz{ \draw[-{Latex[length=2mm, width=2mm]},  ->,>=stealth](0,0) -- (7mm,0);} }}}

==> figures/fig_sd2.tex <==
\newpage
\begin{figure}[!h]
\centering
\execution{2}{
\figev{1}{\acq(\ell_1)}
\figev{1}{\acq(\ell_2)}
\figev{1}{\acq(\ell_3)}
\figev{1}{\wt(x)}
\figev{1}{\rel(\ell_3)}
\figev{1}{\rel(\ell_2)}
\figev{1}{\acq(\ell_4)}
\figev{1}{\rel(\ell_4)}
\figev{1}{\wt(y)}
\figev{1}{\rel(\ell_1)}
\figev{2}{\acq(\ell_2)}
\figev{2}{\wt(x)}
\figev{2}{\rel(\ell_2)}
\figev{2}{\acq(\ell_1)}
\figev{2}{\rel(\ell_1)}
\figev{2}{\acq(\ell_4)}
\figev{2}{\acq(\ell_3)}
\figev{2}{\rd(x)}
\figev{2}{\rel(\ell_3)}
\figev{2}{\rd(y)}
\figev{2}{\rel(\ell_4)}
%\orderedge{1}{6}{0.4}{2}{18}{-0.4}
}
\caption{
The trace has no predictable race or deadlock.
SDP makes one cross-thread ordering $e_6\sdp{\tr} e_{18}$, leaving
$e_9$ and $e_{20}$ unordered.
These two events are not protected by the same lock, so they constitute an SDP-race.
}
\end{figure}
\newpage

==> figures/fig_space_lowerboun2.tex <==
\begin{figure}
\execution{2}{
\figev{1}{\acq( b_1)}
\figev{1}{\acq( b_2)}
\figev{1}{\wt_1(x)}
\figev{1}{\rel( b_2)}
\figev{1}{\rel( b_1)}
\figev{1}{\acq( a_1)}
\figev{1}{\acq( b_2)}
\figev{1}{\rd_2(x)}
\figev{1}{\rel( b_2)}
\figev{1}{\rel( a_1)}
\figev{1}{\acq( a_2)}
\figev{1}{\acq( b_1)}
\figev{1}{\rd_3(x)}
\figev{1}{\rel( b_1)}
\figev{1}{\rel( a_2)}
\figev{1}{\acq( a_1)}
\figev{1}{\acq( a_2)}
\figev{1}{\wt_4(x)}
\figev{1}{\rel( a_2)}
\figev{1}{\rel( a_1)}
\figev{2}{\acq(a_1)}
\figev{2}{\acq( b_2)}
\figev{2}{\rd(x)}
\figev{2}{\rel( b_2)}
\figev{2}{\rel( a_1)}
}
\caption{
Construction of the trace $\tr$ on input $s=1001\#111$.
Observe that $s\not \in \Lang_4$, and $\tr$ does not have a predictable trace.
Modifying a single bit of $s$, we obtain $s'=1001\#111$, which would correspond to trace $\tr'$ identical to $\tr$, except that $\rd_3(x)$ is replaced by $\wt_3(x)$.
Observe that $s'\in \Lang_4$, and $\tr'$ has a predictable, 0-reversal race.
}
\label{fig:space_lowerbound}
\end{figure}

==> figures/fig_space_lowerbound_bk.tex <==
%!TEX root = ../main.tex

\begin{figure}
\execution{2}{
\figev{1}{\acq( b_1)}
\figev{1}{\acq( b_2)}
\figev{1}{\acq( c)}
\figev{1}{\wt_1(x)}
\figev{1}{\rel( c)}
\figev{1}{\rel( b_2)}
\figev{1}{\rel( b_1)}
\figev{1}{\acq( a_1)}
\figev{1}{\acq( b_2)}
\figev{1}{\rd_2(x)}
\figev{1}{\rel( b_2)}
\figev{1}{\rel( a_1)}
\figev{1}{\acq( a_2)}
\figev{1}{\acq( b_1)}
\figev{1}{\rd_3(x)}
\figev{1}{\rel( b_1)}
\figev{1}{\rel( a_2)}
\figev{1}{\acq( a_1)}
\figev{1}{\acq( a_2)}
\figev{1}{\acq( c)}
\figev{1}{\wt_4(x)}
\figev{1}{\rel( c)}
\figev{1}{\rel( a_2)}
\figev{1}{\rel( a_1)}
}
\qquad
\execution{2}{
\figevoffset{24}{2}{\acq( a_1)}
\figevoffset{24}{2}{\acq( a_2)}
\figevoffset{24}{2}{\acq( c)}
\figevoffset{24}{2}{\wt_1(x)}
\figevoffset{24}{2}{\rel( c)}
\figevoffset{24}{2}{\rel( a_2)}
\figevoffset{24}{2}{\rel( a_1)}
\figevoffset{24}{2}{\acq( b_1)}
\figevoffset{24}{2}{\acq( a_2)}
\figevoffset{24}{2}{\rd_2(x)}
\figevoffset{24}{2}{\rel( a_2)}
\figevoffset{24}{2}{\rel( b_1)}
\figevoffset{24}{2}{\acq( b_2)}
\figevoffset{24}{2}{\acq( a_1)}
\figevoffset{24}{2}{\acq( c)}
\figevoffset{24}{2}{\wt_3(x)}
\figevoffset{24}{2}{\rel( c)}
\figevoffset{24}{2}{\rel( a_1)}
\figevoffset{24}{2}{\rel( b_2)}
\figevoffset{24}{2}{\acq( b_1)}
\figevoffset{24}{2}{\acq( b_2)}
\figevoffset{24}{2}{\acq( c)}
\figevoffset{24}{2}{\wt_4(x)}
\figevoffset{24}{2}{\rel( c)}
\figevoffset{24}{2}{\rel( b_2)}
\figevoffset{24}{2}{\rel( b_1)}
}
\caption{
Construction of the trace $\tr$ on input $s=u\#v$ where $u=1001$ and $v=1011$.
Observe that $(e_{15}, e_{40})$ is a \zeroreversal~race, which encodes that $e[3]\neq v[3]$.
}
\label{fig:space_lowerbound}
\end{figure}


==> intro_bk.tex <==
%!TEX root = main.tex

\section{Introduction}
\seclabel{intro}

The verification of concurrent programs is one of the main challenges in formal methods.
Concurrency adds a dimension of non-determinism to program behavior which stems from inter-process communication.
Accounting for such non-determinism during program development is a challenging mental task, making concurrent programming significantly error-prone.
At the same time, bugs due to concurrency are very hard to reproduce manually, 
and automated techniques for doing so are crucial in enhancing productivity of software developers.

Data races are the most common form of concurrency errors.
% The most reliable indicators of errors in concurrency are data races.
A data race (sometimes just called race) occurs when a thread of a multi-threaded 
program accesses a shared memory location 
while another thread is modifying it without proper synchronization. 
The presence of a data race is often symptomatic of a serious bug in the program~\cite{lpsz08},
while they lead to data corruption and compilation errors~\cite{boehmbenign2011,racemob,Narayanasamy2007}, 
and have lead to significant system errors in the past~\cite{SoftwareErrors2009,evil2012}.
Therefore, considerable research has focused on detecting and preventing races in multi-threaded programs.

One of the most popular approaches to race prediction is via dynamic analysis~\cite{fasttrack,bond2010pacer,Pozniansky:2003:EOD:966049.781529}.
Unlike static analysis, dynamic race prediction is performed at runtime. 
Such techniques determine if an observed execution provides evidence for the existence of a \emph{possibly alternate} program execution that can concurrently perform conflicting data accesses~\footnote{Conflicting data accesses are data accesses by two threads to a common memory location such that at least one of them is a write.}.
The underlying principle is that a race is present but ``hidden'' in a large number of different program executions; 
hence techniques that uncover such hidden races can accelerate the
process of debugging concurrent programs.
% have a large overall effect in program correctness by analyzing only few of them.
The popularity of dynamic race prediction techniques further stems
(i)~from their scalability to large production software, and 
(ii)~from their ability to produce only sound error reports.


The most popular dynamic race prediction techniques are 
based on Lamport's happens-before partial order~\cite{lamport1978time}. 
These techniques scan the input trace, determine happens-before orderings on-the-fly, 
and report a race on a pair of conflicting data accesses if they are \emph{unordered} by happens-before. 
This approach is sound, in that the presence of unordered conflicting data accesses ensures the existence of an execution with a race. 
While happens-before based analysis fails to predict races in various cases~\cite{cp2012}, 
its wide deployment is based on the fact that the algorithm is fast, single pass, and runs in linear time. 
The principle that forms the basis of its efficiency is the following.
When reasoning about alternate executions, happens-before analysis does not consider any execution in which the order of synchronization primitives is reversed from that in the observed execution. 
We call such alternate executions \emph{sync(hronization)-reversal free executions}~\footnote{Precise definition of such executions given in \secref{zero_reversals}.} in this paper. 
Other, more powerful race prediction techniques~\cite{cp2012,rv2014,Huang2016,Roemer18,Bond2019,PavlogiannisPOPL20} sacrifice this principle and consider alternate executions that are not \zeroreversal free.
Naturally, this typically results in performance degradation, as the problem is in general $\NP$-hard~\cite{Mathur20},
and considerable efforts are made towards improving the scalability of such techniques~\cite{Roemer20,roemeronline2019}.



\input{figures/compare-hb}
Although happens-before only detects races whose exposure preserves the ordering of synchronization primitives, it can still miss simple races that adhere to this pattern.
For example, consider the trace $\tr_{\two}$ shown in \figref{hb-misses-race}. 
Let us name the events of this trace based on the order in which they appear in the trace; thus, $e_i$ denotes the $i^\text{th}$ event of the trace. 
Here, the partial order happens-before orders the 
first $\wt(x)$ (event $e_1$) and the last $\wt(x)$ (event $e_6$), and therefore, does not detect any race in this execution. However events $e_1$ and $e_6$ are in race. This can be exposed by the alternate execution shown in \figref{ZR-race-missed-by-HB}, which is obtained by dropping the critical section of lock $\lk$ performed by thread $t_1$. 
Notice that the order of synchronization events (namely, $\acq(\lk)$ and $\rel(\lk)$ events) \emph{that appear in the trace} of \figref{ZR-race-missed-by-HB}, are in the same order as in the trace of \figref{hb-misses-race}, and hence this is a sync-reversal free execution.
Thus, the notion of sync-reversal freeness captures races beyond standard happens-before races.

Another important limitation of happens-before and virtually all partial-order methods~\cite{wcp2017,shb2018,Roemer18,Roemer20,cp2012} is highlighted in \figref{predictable-race-intro}.
The trace $\tr_\one$ has a race between $e_1$ and $e_6$, both conflicting on variable $x$.
Notice, however, that the intermediate event $e_3$ also accesses $x$, but is not in race wither either $e_1$ or $e_6$.
Partial-order methods for race prediction are limited to capturing races \emph{only between successive} conflicting accesses.
Hence, distant races that are interjected with intermediate, conflicting but non-racy events are missed by such methods.
On the other hand, sync-reversal freeness is not bound to such limitations: $(e_1, e_6)$ is characterized as a race under this criterion, regardless of the intermediate, non-racy $e_3$, exposed by a witness that omits the critical section on lock $\lk$ in the thread $t_1$.



\Paragraph{Our Contributions.}
Motivated by observations like the above, our contributions are as follows.
\begin{compactenum}
\item 
We introduce the novel notion of \emph{sync(hronization)-reversal free} races.
This is a \emph{sound} notion of predictable races, and it \emph{strictly subsumes} the standard notion of happens-before races.
Moreover, it characterizes races between events that can be arbitrarily far apart in the input trace, as opposed to happens-before and other partial-order methods that only characterize races between \emph{successive} conflicting accesses.
Our notion is applicable to all concurrency settings, and interestingly, it is also \emph{complete} for systems with synchronization-deterministic concurrency~\cite{Bocchino09,Cui15,Aguado18,Zhao19}.
\item 
We develop an efficient, single-pass, nearly linear-time algorithm $\ZeroRevAlgo$
that, given a trace $\tr$, detects whether $\tr$ contains a sync-reversal-free race.
In fact, our algorithm  soundly reports \emph{all} events $e_2$ which are in a sync-reversal-free race with an event $e_1$ that appears earlier in $\tr$.
Given $\NumEvents$ events in $\tr$, our algorithm spends $\Otilde(N)$ time, where $\Otilde$ hides factors poly-logarithmic in $\NumEvents$, when other parameters of the input (e.g., number of threads) are $\Otilde(1)$.
\item 
Although our algorithm performs a single pass of the trace, in the worst case, it might use space that is nearly linear in the length of the trace, i.e., $\Otilde(\NumEvents)$ space.
Hence follows a natural question: is there an efficient algorithm for sync-reversal free race prediction that uses considerably less space?
We answer this question in negative, by showing that  \emph{any} single-pass algorithm for detecting even a single sync-reversal free race must use nearly linear space.
Hence, our algorithm $\ZeroRevAlgo$ has nearly optimal performance in both time and space.
\item 
We next study the complexity of race prediction with respect to the number of synchronization reversals that might occur when constructing a witness that exposes the race.
In the case of synchronization via locks, this number corresponds to the number of critical sections whose order is reversed in the witness trace.
We prove that the problem of predicting races which can be witnessed by \emph{a single} reversal (of two critical sections) is $\NP$-complete and even $\W{1}$-hard when parameterized by the number of threads.
Thus, sync-reversal freeness characterizes \emph{exactly} the tractability boundary of race prediction, and our algorithm is nearly \emph{optimal} for the tractable side.
Moreover, our result shows that \emph{any level} of synchronization suffices to make the problem of race prediction as hard as in the general case, improving a recent result of~\cite{Mathur20}.
\item 
Finally, we have implemented our race prediction algorithm $\ZeroRevAlgo$ and evaluated its performance on standard benchmarks from the literature.
Our results show that sync-reversal freeness characterizes many races that are missed by state-of-the-art methods,
and $\ZeroRevAlgo$ successfully detects them.
\end{compactenum}



==> macros.tex <==
%!TEX root = main.tex

\makeatletter
\newcommand{\pnrelbar}{%
\linethickness{\dimen2}%
\sbox\z@{$\m@th\prec$}%
\dimen@=1.1\ht\z@
\begin{picture}(\dimen@,.4ex)
\roundcap
\put(0,.2ex){\line(1,0){\dimen@}}
\put(\dimexpr 0.5\dimen@-.2ex\relax,0){\line(1,1){.4ex}}
\end{picture}%
}

\newcommand{\precneq}{\mathrel{\vcenter{\hbox{\text{\prec@neq}}}}}
\newcommand{\prec@neq}{%
\dimen2=\f@size\dimexpr.04pt\relax
\oalign{%
\noalign{\kern\dimexpr.2ex-.5\dimen2\relax}
$\m@th\prec$\cr
\noalign{\kern-.5\dimen2}
\hidewidth\pnrelbar\hidewidth\cr
}%
}
\makeatother

\newenvironment{myparagraph}[1]{\vspace*{0.1in}\noindent{\bf #1.}}{}

\SetInd{0.3em}{0.2em}


\newcommand{\ZeroRevAlgo}{\textsf{SyncP}\xspace}
% Labels and references
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\exlabel}[1]{\label{ex:#1}}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\problabel}[1]{\label{prob:#1}}
\newcommand{\probref}[1]{Problem~\ref{prob:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\corlabel}[1]{\label{cor:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\itmlabel}[1]{\label{itm:#1}}
\newcommand{\itmref}[1]{\ref{itm:#1}}
\newcommand{\equlabel}[1]{\label{eq:#1}}
\newcommand{\equref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
% \newcommand{\appref}[1]{ the Appendix}
\newcommand{\algolabel}[1]{\label{app:#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{app:#1}}
\newcommand{\linelabel}[1]{\label{line:#1}}
\newcommand{\lineref}[1]{Line~\ref{line:#1}}
\newcommand{\linerangeref}[2]{Lines~\ref{line:#1}-\ref{line:#2}}
\newcommand{\secrangeref}[2]{Sections~\ref{sec:#1}-\ref{sec:#2}}

\newcommand{\setofthreads}{\mathsf{Thr}}
\newcommand{\threads}[1]{\setofthreads_{#1}}
\newcommand{\locks}[1]{\mathsf{Locks}_{#1}}
\newcommand{\vars}[1]{\mathsf{Vars}_{#1}}
\newcommand{\events}[1]{\mathsf{Events}_{#1}}
\newcommand{\wevents}[1]{\mathsf{WEvents}_{#1}}
%\newcommand{\reads}[1]{\mathsf{Reads}_{#1}}
%\newcommand{\writes}[1]{\mathsf{Writes}_{#1}}
\newcommand{\br}{\mathtt{br}}
\newcommand{\Reads}[1]{\mathsf{Rds}(#1)}
\newcommand{\Writes}[1]{\mathsf{Wts}(#1)}
\newcommand{\accesses}[1]{\mathsf{Accesses}_{#1}}
\newcommand{\acquires}[1]{\mathsf{Acquires}_{#1}}
\newcommand{\releases}[1]{\mathsf{Releases}_{#1}}
\newcommand{\forks}[1]{\mathsf{Forks}_{#1}}
\newcommand{\joins}[1]{\mathsf{Joins}_{#1}}
% \renewcommand{\next}[1]{\mathsf{next}_{#1}}
\newcommand{\match}[1]{\mathsf{match}_{#1}}
\newcommand{\lheld}[1]{\mathsf{locksHeld}_{#1}}
% \newcommand{\last}[1]{\mathsf{last}_{#1}}
\newcommand{\last}[2]{\mathsf{last}^{#1}_{#2}}
\newcommand{\RF}{\operatorname{RF}}
\newcommand{\Otilde}{\widetilde{O}}

\newcommand{\acq}{\mathtt{acq}}
\newcommand{\rel}{\mathtt{rel}}
\newcommand{\rd}{\mathtt{r}}
\newcommand{\wt}{\mathtt{w}}
\newcommand{\fork}{\mathtt{fork}}
\newcommand{\join}{\mathtt{join}}
% \newcommand{\trbegin}{\rhd}
% \newcommand{\trend}{\lhd}
% \newcommand{\trbeginfig}{\texttopcorner\textcorner}
% \newcommand{\trbeginfig}{\;\raisebox{1.3mm}{\rule{0.4pt}{1.14mm}\raisebox{1mm}{\rule{4mm}{0.4pt}}\rule{0.4pt}{1.14mm} } }
% \newcommand{\trendfig}{\;\raisebox{-0.075mm}{\rule{0.4pt}{1.14mm}\rule{4mm}{0.4pt}\rule{0.4pt}{1.14mm} } }
% \newcommand{\trbegintext}{\;\raisebox{0mm}{\rule{1pt}{1.35mm}\raisebox{1mm}{\rule{3mm}{1pt}}\rule{1pt}{1.35mm} } }
% \newcommand{\trendtext}{\;\raisebox{-0.075mm}{\rule{1pt}{1.35mm}\rule{3mm}{1pt}\rule{1pt}{1.35mm} } }
% \newcommand{\trbegin}{{\protect\trbegintext}\!}
% \newcommand{\trend}{{\protect\trendtext}\!}
\newcommand{\trbegin}{\rhd}
\newcommand{\trend}{\lhd}
\newcommand{\trbeginfig}{\rhd}
\newcommand{\trendfig}{\lhd}
\newcommand{\sync}{\mathtt{sync}}
\newcommand{\lk}{\ell}
\newcommand{\ev}[1]{\langle #1\rangle}
\newcommand{\tr}{\sigma}
\newcommand{\conf}{\asymp}
\newcommand{\comp}{\circ}
\newcommand{\wrap}{\mathtt{wrap}}
\newcommand{\clear}{\mathtt{clear}}
\newcommand{\src}{\mathtt{src}}
\newcommand{\thread}{t}
\newcommand{\ThreadOf}[1]{\operatorname{thr}(#1)}
\newcommand{\op}{\mathsf{op}}
\newcommand{\OpOf}[1]{\operatorname{op}(#1)}
\newcommand{\trnsc}{\mathsf{txn}}
\newcommand{\crit}[1]{\mathsf{CS}_{#1}}
\newcommand{\addfresh}{\mathsf{addFresh}}
\newcommand{\W}[1]{\operatorname{W[#1]}}
\newcommand{\NP}{\operatorname{NP}}
\newcommand{\Lang}{\mathcal{L}}
\newcommand{\EQ}{\mathcal{L'}}
\newcommand{\Transducer}{\mathcal{A}}

\newcommand{\Paragraph}[1]{\smallskip\noindent{\bf #1}}
\newcommand{\SubParagraph}[1]{\smallskip\noindent{\em #1}}
\newcommand{\RFPoset}{\mathcal{P}}
\newcommand{\RFPosetQ}{\mathcal{Q}}
\newcommand{\RFPosetS}{\mathcal{S}}
\newcommand{\Unordered}[4]{#1\parallel^{#2}_{#3} #4}
\newcommand{\Ordered}[4]{#1 \not \parallel^{#2}_{#3} #4}
\newcommand{\Project}{|}
\newcommand{\Refines}{\sqsubseteq}
\newcommand{\SeqTrace}{\pi}
\newcommand{\ov}{\overline}
\newcommand{\ReadTriplets}[1]{\mathsf{Triplets(#1)}}
\newcommand{\DistinguishedTriplet}{\lambda}
\newcommand{\NumAcquires}{\mathcal{A}}
\newcommand{\NumVariables}{\mathcal{V}}
\newcommand{\NumThreads}{\mathcal{T}}
\newcommand{\NumEvents}{\mathcal{N}}
\newcommand{\NumLocks}{\mathcal{L}}

\newcommand{\NumRedEvents}{\ov{\mathcal{N}}}
\newcommand{\NumRedLocks}{\ov{\mathcal{L}}}
\newcommand{\NumRedAcquires}{\ov{\mathcal{A}}}
\newcommand{\NumRedVariables}{\ov{\mathcal{V}}}
\newcommand{\NumRedThreads}{\ov{\mathcal{T}}}


\newcommand{\set}[1]{\{#1\}}
\newcommand{\setpred}[2]{\{#1 \,|\, #2\}}
\newcommand{\tuple}[1]{\langle #1 \rangle}

\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
<5> <6> <7> <8> <9> <10> gen * mathb
<10.95> mathb10 <12> <14.4> <17.28> <20.74> <24.88> mathb12
}{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}
% \DeclareMathSymbol{\sqsubsetneq}    {3}{mathb}{"88}
% \DeclareMathSymbol{\varsqsubsetneq} {3}{mathb}{"8A}
% \DeclareMathSymbol{\varsqsubsetneqq}{3}{mathb}{"92}
\DeclareMathSymbol{\sqsubsetneq}    {3}{mathb}{"8A}

\newcommand{\ord}[2]{\leq^{#1}_{\mathsf{#2}}}
\newcommand{\notord}[2]{{\not\leq}^{#1}_{\mathsf{#2}}}
\newcommand{\strictord}[2]{<^{#1}_{\mathsf{#2}}}
\newcommand{\trord}[1]{\leq^{#1}_{\mathsf{tr}}}
\newcommand{\stricttrord}[1]{<^{#1}_{\mathsf{tr}}}
\newcommand{\tho}[1]{\leq^{#1}_{\mathsf{TO}}}
\newcommand{\TO}{TO}
\newcommand{\stricttho}[1]{<^{#1}_{\mathsf{TO}}}
\newcommand{\nottho}[1]{\not\leq^{#1}_{\mathsf{TO}}}
% \newcommand{\stricttrord}[1]{<^{#1}_{\mathsf{tr}}}
\newcommand{\hb}[1]{\leq^{#1}_{\mathsf{HB}}}
\newcommand{\sdp}[1]{\leq^{#1}_{\mathsf{SDP}}}
\newcommand{\chb}[1]{\leq^{#1}_{\mathsf{CHB}}}
%\newcommand{\thb}[1]{<^{#1}_{\mathsf{THB}}}
\newcommand{\thb}[1]{\lessdot^{#1}_{\mathsf{Txn}}}
% \newcommand{\pth}[1]{\stackrel{*, #1}{\longrightarrow}}
\newcommand{\pth}[1]{\stackrel{*}{\longrightarrow_{#1}}}
\newcommand{\nedg}[1]{\lessdot^{#1}_{\mathsf{E}}}
\newcommand{\cp}[1]{\leq^{#1}_{\mathsf{CP}}}
\newcommand{\wcp}[1]{\leq^{#1}_{\mathsf{WCP}}}
\newcommand{\shb}[1]{\leq^{#1}_{\mathsf{SHB}}}
\newcommand{\notwcp}[1]{\not\leq^{#1}_{\mathsf{WCP}}}
\newcommand{\notsdp}[1]{\not\leq^{#1}_{\mathsf{SDP}}}
\newcommand{\strictwcp}[1]{\prec^{#1}_{\mathsf{WCP}}}
\newcommand{\strictshb}[1]{\strictord{#1}{\mathsf{SHB}}}
\newcommand{\ccp}[1]{\leq^{#1}_{\mathsf{DCP}}}
\newcommand{\notccp}[1]{\not\leq^{#1}_{\mathsf{DCP}}}
\newcommand{\strictccp}[1]{\prec^{#1}_{\mathsf{DCP}}}
\newcommand{\conc}[2]{\,||^{#1}_{\mathsf{#2}}\,}
\newcommand{\wcpconc}[1]{\,||^{#1}_{\mathsf{WCP}}\,}
\newcommand{\ccpconc}[1]{\,||^{#1}_{\mathsf{DCP}}\,}
\newcommand{\prev}[1]{\textsf{prev}_{#1}}

\newcommand{\ccprank}[2]{\mathsf{rank}_\mathsf{DCP}^{#1}(#2)}
\newcommand{\wcprank}[2]{\mathsf{rank}_\mathsf{WCP}^{#1}(#2)}

\newcommand{\synctr}[1]{\mathsf{syncTrace}(#1)}
\newcommand{\unsynctr}[1]{\mathsf{unSyncTrace}(#1)}
\newcommand{\synctrev}[2]{\mathsf{syncTrace}^{#2}(#1)}
\newcommand{\freshvar}{\mathsf{fvar}}
\newcommand{\fsync}{\mathsf{first}\sync}
\newcommand{\lsync}{\mathsf{last}\sync}

\newcommand{\lw}[1]{\mathsf{lw}_{#1}}
\newcommand{\RFTrace}[1]{\lw{#1}}
\newcommand{\proj}[2]{#1|_{#2}}

\newcommand{\rtext}[1]{\textcolor{orange}{\sout{#1}}}
\newcommand{\atext}[1]{\textcolor{blue}{#1}}
\newcommand{\qtext}[1]{\textcolor{green}{#1}}

\newcommand{\Andreas}[1]{\textcolor{blue}{AP:~#1}}
\newcommand{\ucomment}[1]{\textcolor{red}{#1}}
\newcommand\mycommfont[1]{\ttfamily{#1}}
% \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\newcommand{\cre}{\mathsf{CR}}

\renewcommand{\emptyset}{\varnothing}

%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
% \newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
% \newtheorem{observation}{Observation}

% \theoremstyle{remark}
% \newtheorem{remark}{Remark}

\newcommand{\closurefun}{\texttt{ComputeSPIdeal}\xspace}
\newcommand{\racefun}{\texttt{checkRace}\xspace}


\input{exec_macros}
\input{pseudocode_macros}

% \newcommand{\trzero}{\rho_1}
% \newcommand{\trone}{\rho_2}
% \newcommand{\trtwo}{\rho_3}
% \newcommand{\trthree}{\rho_4}
% \newcommand{\trfour}{\rho_8}
% \newcommand{\trfive}{\rho_9}
% \newcommand{\trsix}{\rho_6}
% \newcommand{\trseven}{\rho_7}
% \newcommand{\treight}{\rho_5}
% \newcommand{\trnine}{\rho_{10}}
% \newcommand{\trten}{\rho_{11}}

% \newcommand{\nest}[2]{\mathtt{nest}(#1\!\rightarrow\! #2)}
\newcommand{\nest}[2]{\mathtt{nest}(#1,#2)}
% \newcommand{\figevnest}[3]{\figev{#1}{ \nest{#2}{#3} } }
\newcommand{\figevnest}[3]{ \figev{#1}{\acq(#2)}\figev{#1}{\acq(#3)}\figev{#1}{\rel(#3)}\figev{#1}{\rel(#2)} }

\newcommand{\nats}{\mathbb{N}}
\newcommand{\toolname}{\textsc{RAPID}\xspace}
\newcommand{\lhist}{\mathsf{History}}

\newcommand{\djitp}{\textsc{Djit}+}

% \newcommand{\vc}[1]{\!\texttt{#1}\!}
\newcommand{\vc}[1]{$\langle${\texttt{#1}}$\rangle$}



\newcommand{\ZRClosure}[1]{\mathsf{SPClosure}_{#1}}
\newcommand{\ZRIdeal}[1]{\mathsf{SPIdeal}_{#1}}
\newcommand{\TOOClosure}[1]{\mathsf{TLClosure}_{#1}}

%%%%%%%%%% Trace numbers %%%%%%%%%%
\newcounter{count}

\newcommand\generator[1]%
{%
  \stepcounter{count}%
  \expandafter\edef\csname#1\endcsname{\thecount}%
}

\generator{two}
\generator{one}
\generator{exampleone}
\generator{exampletwo}
\generator{examplethree}
\generator{examplefour}
\generator{three}
\generator{four}
\generator{five}
\generator{six}




==> pseudocode_macros.tex <==
%!TEX root = main.tex

%%%%%% Macros for algo %%%%%%%%
\SetKwProg{myfun}{function}{}{}
\SetKwProg{myhandler}{handler}{}{}
\SetKwFunction{init}{Initialization}
% \SetKwFunction{fixpoint}{ComputeLCClosure}
\SetKwFunction{fixpoint}{ComputeSPIdeal}
\SetKwFunction{maxLB}{maxLowerBound}
\SetKwFunction{checkRace}{checkRace}
\SetKwFunction{rdhandler}{read}
\SetKwFunction{wthandler}{write}
\SetKwFunction{acqhandler}{acquire}
\SetKwFunction{relhandler}{release}
\SetKwInput{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKw{Let}{let}
\SetKw{Break}{break}
\SetKw{NOT}{not}
\SetKw{declare}{declare}
\SetKw{exit}{exit}
\SetKwFor{Foreach}{for each}{}{}%
\DontPrintSemicolon
% \newcommand{\ideal}{\mathsf{I}}

\newcommand{\AcqLst}{\mathsf{CSHist}}
\newcommand{\AccLst}{\mathsf{AccessHist}}

\newcommand{\mx}{\sqcup}
\newcommand{\cle}{\sqsubseteq}
\newcommand{\Cc}{\mathbb{C}}
\newcommand{\LW}{\mathbb{LW}}
\newcommand{\Ii}{\mathbb{I}}
\newcommand{\gId}{\mathbbm{g}}
\newcommand{\lastGID}{\gId\mathsf{\_max}}
\newcommand{\lastRelTime}{\mathsf{RelTime\_max}}

\newcommand{\view}[3]{{#1}_{#2}^{#3}}

\renewcommand{\nil}{\mathtt{NIL}}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother
\newcommand{\apicall}[3]{{#1}\bigcdot{\textup{\texttt{#2(#3)}}}}
\newcommand{\first}[1]{\apicall{#1}{first}{}}
\newcommand{\removeFirst}[1]{\apicall{#1}{removeFirst}{}}
\newcommand{\isEmpty}[1]{\apicall{#1}{isEmpty}{}}
\newcommand{\lst}[1]{\apicall{#1}{last}{}}
\newcommand{\addLst}[2]{\apicall{#1}{addLast}{#2}}
\newcommand{\updateRel}[2]{\apicall{#1}{updateRelease}{#2}}

\newcommand{\true}{\top\!\!\!\!\top}
\newcommand{\false}{\bot\!\!\!\!\bot}

==> ptime.tex <==
\subsection{Efficient Dynamic Data Race Prediction}\label{subsec:ptime}


\begin{proof}[Proof of \thmref{dichotomy} (upper bound).]

\end{proof}

==> space_lowerbound2.tex <==
%!TEX root = main.tex

\subsection{Linear Space Lower Bound}\label{subsec:space_lowerbound}


\Paragraph{The language $\Lang_n$.}
Given a natural number $n$, we define the language
\[
\Lang_n =\{u\#\ell\colon u\in \{0,1\}^n \text{ and } \ell\in \{1\}^{\leq n} \text{ and } u[i]=1 \text{ where $i$ is the number encoded by $\ell$ in unary} \}\ .
\] 

\smallskip
\begin{restatable}{lemma}{lemlangnlowerbound}\label{lem:langnlowerbound}
Any streaming algorithm that recognizes $\Lang_n$ uses $\Omega(n)$ space.
\end{restatable}
\begin{proof}
Assume towards contradiction otherwise, i.e., there is an algorithm that uses $o(n)$ space.
Then, there exist two distinct $n$-bit strings $u_1$, $u_2$, such that the algorithm is in the same state after parsing $u_1$ and $u_2$.
Let $\ell$ be the binary encoding of a number such that $u_1[\ell]\neq u_2[\ell]$.
Observe that $u_i\#\ell \in \Lang_n$ for exactly one $i\in [2]$.
On the other hand, the algorithm gives the same answer on the two inputs for each $i\in[2]$.
Hence the algorithm cannot recognize $\Lang_n$, a contradiction.
\end{proof}

\input{figures/fig_space_lowerbound}
\Paragraph{Reduction from $\Lang_n$ recognition to dynamic race prediction with 0-reversals.}
Consider the language $\Lang_n$ for some $n$.
We describe a transducer $\Transducer_n$ such that, on input a string 
$u\#\ell$, the output $\Transducer_n(u\#\ell)$ is a trace $\tr$ with $2$ threads, $O(n\cdot \log n)$ events, $2\cdot \log n$ locks and a single variable such that the following hold.
\begin{compactenum}
\item If $u\#\ell\not \in \Lang_n$, then $\tr$ has no predictable race.
\item If $u\#\ell \in \Lang_n$, then $\tr$ has a single predictable race, which is a 0-reversal race.
\end{compactenum}
Moreover, $\Transducer_n$ uses $O(\log n)$ working space.
The transducer $\Transducer_n$ uses a single variable $x$ and two sets of locks $A=\{ a_1,\dots, a_{\log n} \}$ and $B=\{b_1, \dots, b_{\log n} \}$.
The trace $\tr$ consists of two threads, $\thread_1$ and $\thread_2$, which encode the bits of $u$ and $\ell$, respectively.
See \cref{fig:space_lowerbound} for an illustration.

We first describe $\thread_1$.
For every $i\in [n]$, $\thread_1$ contains an event $e_i(x)$, which is a write event $\wt_{i}(x)$ if $u[i]=1$, otherwise it is a read event $\rd_i(x)$.
The events $e_i$ are surrounded by locks from $A$ and $B$ arbitrarily, as long as the following property is guaranteed.
For any $i<j$, we have
\begin{align*}
\lheld{\tr}(e_j)\cap A \not \subseteq \lheld{\tr}(e_i) \cap A \quad \text{ and }\quad \lheld{\tr}(e_i)\cap B \not \subseteq \lheld{\tr}(e_j) \cap B\ .
\end{align*}
The property can be easily met, e.g., by making $\Transducer_n$ perform a breadth-first traversal of the subset-lattice of $A$ (resp., $B$)
starting from the top (resp., bottom).
Given the current $i$, the transducer surrounds $e_i$ with the locks of the current element in the corresponding lattice. 

We now describe $\thread_2$.
The transducer reads $\ell$,
and outputs the event $\rd(x)$, surrounded by a critical section on every lock of the set $(A\cup B )\setminus \lheld{e_{i}}$, where $i$ the number represented by $\ell$ in unary.
Similarly to $\thread_1$, this can be easily achieved by a breadth-first traversal in the two subset-lattices.


\smallskip
\begin{restatable}{lemma}{lemlangn_reordering}\label{lem:langn_reordering}
There exists a correct reordering $\tr^*$ of $\tr$ in which $e_i(x)$ and $\rd$ are enabled iff $\ell$ is the unary representation of $i$.
Moreover, if such a correct reordering exists, then it is a 0-reversal reordering.
\end{restatable}
\begin{proof}
By construction, if $\ell$ is the unary representation of $i$, then $\lheld{\tr}(e_i)\cap \lheld{\tr}(\rd)=\emptyset$, hence we can construct the correct reordering $\tr^*$ by executing $\thread_1$ until $e_i$ and then executing $\thread_2$ until $\rd$.
Observe that $\tr^*$ is a 0-reversal reordering.
For the inverse direction, by construction, recall that we have $(A\cup B )\setminus \lheld{e_{i}}$.
Hence, it suffices to show that for every $j\neq i$, we have
\begin{align*}
((A\cup B)\setminus \lheld{\tr}(e_i)) \cap \lheld{\tr}(e_j) \neq \emptyset\ .
\end{align*}
We split cases based on $j$.
\begin{compactenum}
\item[$j>i$.] By construction, we have $\lheld{\tr}(e_j)\cap A \not \subseteq \lheld{\tr}(e_i) \cap A$.
Thus, there exists a lock $a\in A$ with $a\in \lheld{\tr}(e_j)\setminus \lheld{\tr}(e_i)$.
Observe that $a\in (A\setminus \lheld{\tr}(e_i)) \cap \lheld{\tr}(e_j)$, as desired.
\item[$j<i$.] The argument is similar to the previous case, with $A$ replaced by $B$.
\end{compactenum}

The desired result follows.
\end{proof}

\smallskip
\begin{restatable}{lemma}{lemlangncorrectness}\label{lem:langn_correctness}
The following assertions hold.
\begin{compactenum}
\item If $u\#\ell\not \in \Lang_n$, then $\tr$ has no predictable race.
\item If $u\#\ell \in \Lang_n$, then $\tr$ has a single predictable race, which is a 0-reversal race.
\end{compactenum}
\end{restatable}
\begin{proof}
By \cref{lem:langn_reordering}, there exists exactly only correct reordering $\tr^*$ of $\tr$ in which $e_i$ and $\rd$ are enabled, namely, for $i$ being the number represented by $\ell$ in unary.
In addition, $\tr^*$ is a 0-reversal reordering.
Observe that $\tr$ has a predictable race iff $\tr^*$ has a race.
In turn, this holds iff $e_i$ is a write event $\wt(x)$.
By construction, $e_i$ is a write event iff $u[i]=1$, i.e., iff $u\#\ell \in \Lang_n$.

The desired result follows.
\end{proof}



\smallskip
\begin{restatable}{theorem}{thmspacelowerbound}\thmlabel{space_lowerbound}
Any algorithm for the decision problem of dynamic race prediction with 0-reversals on traces with $2$ threads, $n$ events and $\Omega(\log n)$ locks uses $\Omega(n/\log n)$ space.
\end{restatable}
\begin{proof}
Consider any such algorithm $A_1$ executed in the family of traces $\tr$ constructed in our above reduction.
Let $m=n/\log n$,
and assume towards contradiction that $A_1$ uses $o(m)$ space.
Then we can pair $A_1$ with the transducer $\Transducer_{m}$, and obtain a new algorithm $A_2$ for recognizing $\Lang_{m}$.
Since $\Transducer_{m}$ uses $O(\log m)$ space, the space complexity of $A_2$ is $o(m)$.
However, this contradicts \cref{lem:langnlowerbound}.
The desired result follows.
\end{proof}

\smallskip
\begin{corollary}
Any algorithm for the problem with a space complexity that does not depend on $n$ (like $\mathsf{HB}$) must have exponential dependency on $d$.
\end{corollary}



==> trace1.tex <==
%!TEX root = main.tex

\begin{figure}[h]
\centering
\execution{3}{
  \figev{1}{\trbeginfig}
  \figev{1}{\wt(x)}
  \figev{2}{\trbeginfig}
  \figev{2}{\rd(x)}
  \figev{2}{\trendfig}
  \figev{3}{\trbeginfig}
  \figev{3}{\wt(z)}
  \figev{3}{\trendfig}
  \figev{1}{\rd(z)}
  \figev{1}{\trendfig}
  \orderedge{1}{2}{0.4}{2}{4}{-0.4}
  \orderedge{3}{7}{-0.43}{1}{9}{0.4}
}
\caption{Trace $\rho_1$. Taking $T_i$ to be the transaction of thread $t_i$, we have $T_3 \thb{\rho_1} T_1 \thb{\rho_1} T_2$.}
\figlabel{trace-pred-change}
\end{figure}

